Stabilizing language models under continual learning via condition-anchored distillation

Continual adaptation of language models can change their output distribution on prompts learned earlier, while retaining every old prompt-answer pair may be undesirable or impossible. We study condition-anchored generative distillation (CAGD): retain a small set of old prompts, use a frozen previous model to reconstruct completions and generation states, and match its predictive distributions while learning the next task. The formulation separates three roles that ordinary replay conflates: conditions select the behavior to protect, teacher generations locate relevant states, and soft targets specify how predictions may change. For autoregressive language generation, teacher-rollout distillation admits an exact chain-rule decomposition of sequence divergence. For masked-diffusion language modeling, our implementation directly controls local denoising drift on teacher-generated completions. In continual adaptation of a 219M masked diffusion language model, CAGD reduces four-task final held-out loss from 2.927 to 1.114 in one task order and from 2.168 to 0.891 in exact reverse. The same soft targets lower final average loss by 0.055 over hard replay when teacher-generated support is held identical. The direction persists on fresh facts and natural instructions across SMDM and Qwen3. On GSM8K, Qwen adaptation preserves answer-format compliance, but exact-match retention is seed-mixed at 0.6B and worsens at 1.7B. These results support condition-anchored functional preservation as a common design principle across the tested language-generation objectives.

==> inputs/05-discussion.tex <==
\section{Discussion}

A condition anchor is a behavioral index rather than a compressed old
example: it specifies which conditional distribution should remain stable,
while the temporary teacher reconstructs that distribution.  Hard replay
collapses the teacher to one sequence; \CAGD{} also retains probability mass
over alternatives at visited states.  The matched intervention identifies a
small, seed-consistent benefit from this soft target, although its magnitude
can change once methods induce different teachers and generated support.  The
anchor cache therefore defines the operational scope of retention: behaviors
outside its coverage remain unconstrained, and deployment frequencies or
risks may require the weighting in \eqref{eq:coverage}.

Using the immediately preceding checkpoint keeps \CAGD{} online, but teacher
errors can propagate and repeated greedy generations can narrow support.
The guarantees likewise follow what is actually distilled: sampled AR
next-token kernels admit the exact chain-rule statement, whereas the present
masked-diffusion implementation directly guarantees local denoising stability.
Extending the stronger output-level statement to another sampler requires its
transitions, state visitation, and weights to match the distilled objective.


==> inputs/appdx-audit.tex <==
\section{Artifact Audit and Invalidation}

The geometry submission uses 660 split-sample records: 432 primary records,
216 audited data/objective controls, and 12 dense-slice controls.  Raw outputs
live under \path{runs/r08_split_primary}, \path{runs/r12_audited_controls}, and
\path{runs/r10_attention_split}.  Exact backend replays at both checkpoint scales
match all common metadata and metrics with maximum numerical difference zero.
These records are repeated condition measurements, not 660 independent
replicates; intervals in the main text use the probe-seed mean as their unit.

The confirmatory DLLM submission uses only the R16 validation, confirmation,
four-task, and fresh-fact directories; the exploratory scale extension uses
the separately frozen Qwen continual directories.  All R14/R15 continual outputs are
invalid because their corruption routine forced the first answer token to be
masked when an independent Bernoulli draw was empty.  This changed that
token's marginal probability while retaining the $1/t$ weight.  They also
shared one Python random stream between current and replay minibatches, so GD
changed the current-example sequence.  R16 permits empty masks, separates the
two streams, increases evaluation from 4 to 32 mask replicates, and reruns all
reported continual results.
Each locked long-horizon run snapshots source, dependency, checkpoint,
tokenizer, data, and validation-summary hashes before model loading and checks
the same snapshot again before writing its result; a mid-run artifact change
therefore fails rather than relabeling in-memory code with a later disk hash.

An earlier pilot additionally selected replay rows in file order, giving
per-fact counts 30/30/4/0.  The four-task replacement uses 16/16/16/16 and
audits per-fact hashes.  Because facts 8--23 had already been exposed, the
core comparison is also repeated on the previously unused facts 24--29.  Old
files remain listed in \path{report/INVALIDATED_RESULTS.md} but are not read by
the R16 summarizers.  Earlier geometry r00--r04 artifacts used an incorrect rank-1
Frobenius norm; r05--r06 are same-sample audit-only results.  The complete
rationale is retained in \path{report/INVALIDATED_RESULTS.md} rather than
deleting failed history.

Experiments ran in Python 3.9.25 with PyTorch 2.4.1+cu121 on NVIDIA A100
40GB GPUs.  Model forward/backward uses bfloat16 autocast, cross-entropy logits
and extracted gradient slices use float32, and geometry Gram/reconstruction
algebra uses float64.  The exact interpreter does not resolve flash-attention,
fused dropout-layer-norm, or fused cross-entropy extensions; backend replay
audits therefore bind the results to PyTorch SDPA, the project RMSNorm fallback,
and PyTorch cross-entropy.

The Qwen3 extension contains 132 validation and 36 formal runs across 0.6B,
1.7B, and 4B.  Each result binds the runner, frozen base protocol or 1.7B
addendum, model inventory, data, and selected-lambda artifact by content hash.  The
combined summarizer requires the complete four-method, three-seed matrix at
each scale and recomputes final loss, forgetting, and paired effects.  These
runs used Python 3.11.15, PyTorch 2.7.0+cu128, Transformers 4.57.6, bfloat16
weights, and PyTorch SDPA on the same A100 class.


==> inputs/appdx-continual.tex <==
\section{Continual-Learning Details}

\input{inputs/tables/two_task}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/two_task_confirmation.pdf}
\caption{Two-task confirmation.  Dots are paired seeds; bars are mean
$\pm$ SEM.  GD removes severe sequential forgetting; neither Fisher penalty
provides a repeatable improvement over GD.}
\label{fig:two-task}
\end{figure}

\subsection{Validation sweep and Fisher audit}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/validation_lambda_sweep.pdf}
\caption{Two-task validation on facts 0--3.  Curves show mean $\pm$ SEM and
dots show the three paired seeds.  The minimum mean is selected separately
for each Fisher structure before confirmation or longer-horizon experiments.}
\label{fig:validation}
\end{figure}

At validation, Sequential and GD reach average losses
$1.869_{\pm0.088}$ and $0.298_{\pm0.031}$.  Rank-1+GD is minimized at
$\lambda=10^5$ ($0.263_{\pm0.007}$), whereas Diagonal+GD is minimized at
$\lambda=10^3$ ($0.271_{\pm0.019}$).  The choices are fixed separately rather
than treating a common numeric $\lambda$ as matching implemented weighted
trace.

Across confirmation seeds, the normalized rank-1 coefficient carries 0.642,
0.704, and 0.851 of the diagonal trace, while its absolute coefficient ranges
from $4.82\times10^{-4}$ to $4.49\times10^{-2}$.  This 93-fold scale variation
reinforces that the selected regularizers are fixed recipes, not Fisher
structures matched in implemented weighted trace.  The upstream gradient
clip of 1 is active on
0.976, 0.987, and 0.975 of Task-B steps for GD, Rank-1+GD, and Diagonal+GD;
we retain that faithful optimizer setting and report the clip diagnostic
rather than interpreting raw pre-clip gradient scale as a mechanism result.

\subsection{Four-task audit contract}

\begin{table}[t]
\centering
\caption{Four-task run matrix.  Entries are paired optimization seeds.}
\label{tab:matrix}
\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lccc}
\toprule
Method & Forward & Reverse & Role\\
\midrule
Sequential & 3 & 3 & Forgetting control\\
GD & 3 & 3 & Replay-only control\\
Rank-1 only / Diagonal only & 3 / 3 & -- & Component ablation\\
Rank-1+GD / Diagonal+GD & 3 / 3 & 3 / 3 & Main comparison\\
Joint & 3 & -- & Offline reference\\
\bottomrule
\end{tabular}
\end{table}

The final task set is never used for hyperparameter selection.  Every task's
evaluation mask seed is a function only of optimization seed and canonical
task index, so learned-time and final loss use identical Monte Carlo masks and
the same task remains paired under reversed order.  The primary forgetting
metric is recomputed from raw stage losses by the summarizer.

Each output records 30/10/10 exact train/Fisher/test counts per fact,
selected-row hashes, per-old-task and per-fact replay counts and prompt hashes,
generated replay hashes, Fisher coefficient/trace, raw and weighted EWC loss,
penalty maximum, and final per-task metrics.  The summarizer requires the
predeclared 16/16/16/16 replay split.  Joint training receives the same total
number of optimizer updates as the sequential stream and samples the union of
the four equal-sized task datasets.

\input{inputs/tables/r16_main}
\input{inputs/tables/r16_per_task}
\input{inputs/tables/r16_secondary}
\input{inputs/tables/r16_mechanism}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/multitask_trajectories.pdf}
\caption{Four-task trajectories under the two exact task orders.  Each point
averages the held-out loss of all tasks observed by that stage; error bars are
mean $\pm$ SEM across the three paired optimization seeds.  Because each stage
adds a task to the averaged set, this is a training-dynamics view, not a
standalone forgetting curve; per-task learned-to-final deltas provide the
retention evidence.}
\label{fig:r16-trajectories}
\end{figure}

\subsection{Fresh-fact sensitivity extension}

The fresh-fact sensitivity extension uses the same frozen optimizer, masking,
evaluation, replay, and selected coefficients as the main matrix, but replaces
facts 8--23 with previously unused facts 24--29.  Because only six unexposed
fact groups remained, it has three tasks with two facts each rather than the
main matrix's four tasks with four facts each; it is not a matched replication.
Its two orders are exact reversals, and every method has the same three paired
optimization seeds.

\input{inputs/tables/fresh_main}
\input{inputs/tables/fresh_per_task}
\input{inputs/tables/fresh_secondary}
\input{inputs/tables/fresh_mechanism}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fresh_results.pdf}
\caption{Fresh-fact continual-learning endpoints.  Panels and conventions
match \cref{fig:r16-main}; paired differences below zero favor the method
named first.}
\label{fig:fresh-results}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fresh_trajectories.pdf}
\caption{Fresh-fact trajectories under both exact task orders.  Each point
averages the held-out loss of tasks observed by that stage; error bars are
mean $\pm$ SEM across paired optimization seeds.}
\label{fig:fresh-trajectories}
\end{figure}

\clearpage
\subsection{Full-parameter continual-task Fisher controls}
\label{app:continual-fisher-controls}

\subsubsection{Does the fitted Fisher transfer to held-out continual gradients?}

The packed-text geometry audit and the EWC experiment differ in objective,
data layout, parameter set, and training state.  We therefore ran an
exploratory measurement at the learned Task-A checkpoint of the main forward
stream.  For each of seeds 3407--3409, we reproduced Task-A training, fitted
the operational rank-1 and diagonal tensors on its 40 designated Fisher
rows, and scored them on 40 held-out prompts with independent masks.  Both
passes use the same answer-only objective as continual training and cover all
219,050,496 trainable parameters.  We score exactly the tensors stored by the
continual implementation, without renormalizing the represented direction.

\input{inputs/tables/r18_continual_geometry}

Both calibration-fitted surrogates leave essentially all held-out Fisher
energy unexplained: their mean relative Frobenius errors are
0.9999999957 for rank-1 and 0.99999999999 for diagonal
(\cref{tab:r18-continual-geometry}).  The tiny difference between these two
near-unit errors is not evidence of a structural tie.  Holding only the
calibration direction fixed and refitting its scalar on the test gradients
still gives error $0.999995_{\pm0.000003}$, whereas fitting the best rank-1
matrix to the test Fisher itself gives $0.446_{\pm0.064}$.  Thus the held-out
Fisher can be substantially low-rank, but the direction and scale inferred
from the calibration gradients do not transfer.  The test/calibration loss
ratio ranges from 981 to 3899 (mean 2609), exposing a large shift across the
disjoint templates and realized masks.  This one-task diagnostic closes the
local objective/parameter mismatch in the broad audit; it does not establish
geometry for later tasks, other streams, or a checkpoint population.

\subsubsection{Matched implemented weighted trace and clipping}

The locked R16 EWC multipliers were selected separately for utility, so they do
not isolate Fisher structure.  In a separate exploratory two-task control, we
compare GD, Rank-1+GD, and Diagonal+GD after matching the implemented weighted
trace.  If the stored rank-1 matrix is $\alpha\vu\vu^\top$ and the stored
diagonal is $D$, we fix $\lambda_{\mathrm D}=1000$ and set
\begin{equation}
\lambda_{\mathrm{R1}}
=1000\,\frac{\tr(D)}{\alpha\lVert\vu\rVert_2^2},
\qquad
\tr(\lambda_{\mathrm{R1}}\alpha\vu\vu^\top)
=\tr(\lambda_{\mathrm D}D).
\label{eq:implemented-trace-match}
\end{equation}
The resulting rank-1 EWC multipliers are 2824, 1792, and 1481 across the three
paired seeds.  The model, answer-only Fisher rows, balanced 64-prompt replay,
and 1,000-step Task-A/Task-B stream otherwise match the main forward protocol.
We run both the canonical clip threshold 1 and an inactive threshold $10^6$;
all 18 method--clip--seed cells were fixed before the first result.

\input{inputs/tables/r23_trace_endpoints}
\input{inputs/tables/r23_trace_paired}

With clip 1, Rank-1+GD and Diagonal+GD differ from GD in final average loss by
$-0.040_{\pm0.040}$ and $-0.041_{\pm0.090}$, while their direct difference is
$+0.001_{\pm0.052}$.  Without active clipping, the corresponding increments
over GD reverse to $+0.022_{\pm0.017}$ and $+0.028_{\pm0.035}$, and the direct
rank-1--diagonal difference remains small and seed-dependent
($-0.005_{\pm0.031}$).  Removing clipping lowers final-task loss in every seed
for every method.  For Rank-1+GD and Diagonal+GD it also increases past-task
forgetting in all three seeds, by $+0.132_{\pm0.076}$ and
$+0.127_{\pm0.053}$; GD has no consistent change
($-0.011_{\pm0.186}$).

Trace equality does not equate the penalty encountered along an optimization
trajectory.  Mean weighted EWC is about 24 times larger for rank-1 than for
diagonal with clip 1 and about 10 times larger without clipping
(\cref{tab:r23-trace-endpoints}).  This control therefore finds no stable
structural winner and identifies clipping as part of the observed
retention--acquisition tradeoff.  Matching a single matrix trace does not
match directional stiffness, parameter displacement, or per-step penalty;
with three seeds on one two-task factual stream, these results do not support
a superiority claim.

\subsubsection{Full-parameter 1.14B scale extension}

We predeclared the same two-task implemented weighted-trace comparison at the
1.14B SMDM checkpoint.  All 1,142,367,744 parameters train for 1,000 steps per
task; the 40-row answer-only Fisher, balanced 64-prompt replay, optimizer, and
canonical clip threshold 1 match the 219M control.  The fixed grid contains
GD, Rank-1+GD, and Diagonal+GD at seeds 3407--3409.  Sequential training is not
repeated because this extension asks only about the incremental Fisher
structure beyond the common GD baseline.

\input{inputs/tables/r24_trace_scale}
\input{inputs/tables/r24_trace_paired}

Rank-1+GD minus GD changes final average loss by
$+0.052_{\pm0.061}$: two seeds have small favorable differences
($-0.011$ and $-0.007$), while seed 3407 is $+0.175$.  Its final-task loss is
lower in all three seeds ($-0.044_{\pm0.026}$), but past-task forgetting is
higher on average ($+0.149_{\pm0.147}$), so the acquisition gain does not
produce a stable final-average improvement.  Diagonal+GD has lower final
average loss than GD in all three seeds ($-0.028_{\pm0.008}$).  In the direct
structural comparison, Rank-1+GD has higher final average loss and forgetting
in every seed, with paired means $+0.080_{\pm0.070}$ and
$+0.217_{\pm0.204}$, while its final-task loss is lower in two seeds
(\cref{tab:r24-trace-paired}).

The Fisher scale is highly seed-sensitive.  Although their implemented
weighted traces are matched within each seed, the shared target ranges from
0.145 to 37,149 across seeds, a $2.57\times10^5$-fold span.  The rank-1 mean
weighted EWC component likewise ranges from $2.76\times10^{-6}$ to 141.65,
and its largest adverse endpoint occurs in the high-trace seed; all outcomes
remain in the predeclared summary (\cref{tab:r24-trace-scale}).  Every seed
descriptively favors diagonal on final average loss, but three seeds, one
checkpoint, and one two-task factual stream cannot establish general
diagonal superiority.  The result instead reinforces that trace matching
alone does not control the trajectory-level penalty or remove estimator-scale
instability.

\subsection{Cross-scale continual-learning extension}
\label{app:continual-scale}

We place the full-parameter 219M DLLM result and the autoregressive Qwen3
scale extension in one directional comparison.  All four points use the same
four-task forward stream, three paired seeds, 1,000 updates per task, and the
same definitions of final average held-out loss and past-task forgetting.
The Qwen3-0.6B, Qwen3-1.7B, and Qwen3-4B experiments adapt only the final Transformer block
so that the model, optimizer, frozen GD teacher, and Fisher state fit on one
40GB A100.  For each Qwen scale and Fisher structure, the EWC coefficient is
selected on the disjoint two-task validation stream before the formal run.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/continual_scale.pdf}
\caption{Paired continual-learning effects at the 219M DLLM checkpoint and
three autoregressive Qwen3 scales.  Small dots are the three optimization seeds;
large points and bars are mean $\pm$ SEM.  Negative values favor the method
named first.  Endpoint definitions and task identities match, but DLLM masked
loss and autoregressive answer loss are different objectives; signs support a
qualitative robustness comparison, whereas cross-family magnitudes do not
measure a causal parameter-count effect.}
\label{fig:continual-scale}
\end{figure}

The transferred GD effect has the same direction in all four settings.
Relative to Sequential, GD changes final average loss by
$-1.813_{\pm0.143}$ at 219M and $-1.376_{\pm0.089}$,
$-1.116_{\pm0.064}$, and $-1.199_{\pm0.175}$ at 0.6B, 1.7B, and 4B;
the corresponding forgetting changes are $-1.918_{\pm0.270}$,
$-1.819_{\pm0.108}$, $-1.535_{\pm0.079}$, and $-1.637_{\pm0.209}$.
Every paired seed favors GD on both endpoints in all four settings.

The incremental rank-1 result is not similarly robust.  Rank-1+GD minus GD
changes final average loss by $-0.132_{\pm0.603}$ at 219M, with substantial
seed heterogeneity, but by $+2.213_{\pm0.148}$ at 0.6B,
$+1.341_{\pm0.190}$ at 1.7B, and $+1.382_{\pm0.524}$ at 4B, with no Qwen seed
favoring Rank-1+GD.  Moreover,
its low raw Qwen forgetting accompanies severe failure to acquire the final
task: final-task loss rises from 0.324 to 5.276 at 0.6B, from 0.368 to 5.156
at 1.7B, and from 0.301 to 4.574 at 4B.  Diagonal+GD is worse than GD at 0.6B,
slightly better at 1.7B, and indistinguishable at 4B.  The cross-scale evidence
therefore supports GD as the reliable
forgetting-mitigation component, not a stable incremental benefit from the
rank-1 Fisher penalty.


==> inputs/appdx-geometry.tex <==
\section{Additional Geometry Results}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/finite_sample_null.pdf}
\caption{Isotropic finite-sample null.  Same-sample scoring creates rank-1
wins at low $n/d$; independent-test and population scoring reject the same
surrogate in every simulated setting.}
\label{fig:null}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/geometry_robustness.pdf}
\caption{Calibration size, cell wins, and alignment.  Calibration
mean/top-eigenvector alignment is only moderately associated with held-out
surrogate score.}
\label{fig:geometry-robustness}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{figures/dense_slice_control.pdf}
\caption{Dense attention-projection control.  Diagonal wins all three fixed
mask-condition means on the measured 589,824-parameter slice.}
\label{fig:dense}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/corpus_heatmaps.pdf}
\caption{\textbf{Mask probability.} Matched dataset-plus-preprocessing controls.  A late/high-mask
advantage recurs, but average margins are small and cell rankings vary.}
\label{fig:corpora}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/objective_heatmaps.pdf}
\caption{\textbf{Context mask probability.} Paired all-target versus one-target intervention.  Contexts are
identical, so cell changes arise from supervised-target aggregation; the
grid-average interval still crosses zero.}
\label{fig:objective}
\end{figure}

All reconstruction errors are computed matrix-free.  For
$R=cuu^\top$ and test gradient matrix $G_t$,
\begin{align}
\|\Ftest\|_F^2&=\tr[(G_tG_t^\top/n_t)^2],\\
\langle\Ftest,R\rangle_F&=\frac{c}{n_t}\|G_tu\|_2^2,\\
\|R\|_F^2&=c^2\|u\|_2^4.
\end{align}
The square on $c$ is essential.  Earlier internal artifacts that omitted it
are explicitly invalidated.  The self-check materializes small Fishers and
verifies the rank-1 and diagonal identities plus held-out oracle ordering.


==> inputs/appdx-parameter.tex <==
\subsection{Parameter-Space Baselines}
\label{app:parameter-baselines}

\subsubsection{Elastic Weight Consolidation}

EWC is retained only as a secondary comparison between function-space and
parameter-space preservation \citep{Kirkpatrick2017}.  The reproduced
four-task matrix fitted rank-1 and diagonal empirical-Fisher penalties on
separate old-task examples, with coefficients selected on disjoint validation
facts.  Neither EWC-only method matched the consistency of \CAGD{}:
forward final average loss was $2.189_{\pm0.408}$ for rank-1 EWC and
$3.131_{\pm0.282}$ for diagonal EWC, compared with
$1.114_{\pm0.374}$ for \CAGD{}.
Past-task forgetting is $1.942_{\pm0.460}$ and $2.793_{\pm0.356}$,
and final-task loss is $0.357_{\pm0.046}$ and $0.426_{\pm0.037}$,
respectively.  These EWC-only runs use the forward order.

\subsubsection{Rank-1 and Diagonal Controls}

Adding EWC to \CAGD{} changes retention loss in a scale- and seed-dependent
way.  In a separate two-task control that matched the
implemented weighted trace, rank-1+\CAGD{} minus diagonal+\CAGD{} final loss
was $-0.038_{\pm0.154}$ at 219M with canonical clipping and
$-0.523_{\pm0.298}$ at 1.14B; lower favors the first method.
The latter favors rank-1 in every seed, whereas the 219M contrast is
seed-mixed at both clipping thresholds.  These controls
do not identify a stable Fisher structure and are not part of \CAGD{}
(\cref{tab:r23-trace-paired}).

\input{inputs/tables/r23_trace_paired}


==> inputs/appdx-theory.tex <==
\section{Theory Details}
\label{app:theory}

For $x\sim\mathcal N(0,\sigma^2I)$ and
$g_A(x)=\kappa Bxx^\top$, define the Fisher operator through
$\mathcal F_B[H]=\E[\langle g_A(x),H\rangle_Fg_A(x)]$.  Since
$\langle g_A(x),H\rangle_F=\kappa x^\top B^\top Hx$, Isserlis' identity gives
\begin{equation}
\E[(x^\top Cx)xx^\top]=\sigma^4[\tr(C)I+C+C^\top],
\end{equation}
which yields \cref{eq:fisher-operator} after substituting $C=B^\top H$ and
left-multiplying by $\kappa^2B$ \citep{Isserlis1918}.

For $B=\beta I$, let $C_0=\kappa^2\beta^2\sigma^4$.  The operator acts as
$\mathcal F_B[H]=C_0[\tr(H)I+H+H^\top]$.  On $I$ it has eigenvalue
$C_0(d+2)$; on traceless symmetric matrices it has eigenvalue $2C_0$; and on
antisymmetric matrices it vanishes.  Removing the leading component leaves
$d(d+1)/2-1$ copies of $2C_0$.  Dividing their squared mass by total squared
mass and simplifying gives the residual in \cref{eq:counterexample}.  The
mean gradient $\E[g_A(x)]=\kappa\beta\sigma^2I$ is the leading direction, so
the counterexample does not rely on a poorly chosen rank-1 vector.

At exact convergence $B=0$, every gradient and the Fisher vanish.  There is
then no nontrivial sensitive direction.  The result concerns a finite residual
near an optimum, precisely where EWC estimates curvature.


==> inputs/reproduce.tex <==
\section*{Reproducibility Statement}

All primary geometry rows use disjoint calibration and test gradients.  A
strict geometry manifest verifies the complete grids; source, checkpoint, and
data hashes; held-out oracle ordering; exact paired-mask contracts; and backend
replays.  Invalidated pilot families remain in an explicit ledger and are not
read by the paper figure builder.

The continual runner records checkpoint, tokenizer, reverse-data, source,
dependency, selected-row, replay-prompt, and generated-replay hashes in every
JSON.  Locked-protocol flags reject deviations from exact tasks, per-fact row
counts, training/evaluation settings, methods, or seeds.  The R16 summarizer
accepts only the complete 33-run four-task or 24-run fresh-fact matrix and
recomputes means, paired differences, and forgetting from stage-level metrics.
Commands, environment versions, raw JSON paths, and invalidation decisions
appear in the appendix and repository documentation.


==> inputs/tables/cagd_fresh_components.tex <==
\begin{table}[h]
\centering
\caption{End-to-end replay comparison on the fresh three-task stream
(mean $\pm$ SEM over three seeds).  Methods use their own
evolving teachers and generated completions after they diverge.}
\label{tab:cagd-fresh-components}
\small
\setlength{\tabcolsep}{3.8pt}
\begin{tabular}{ccccc}
\toprule
\tablehead{Method} & \tablehead{Order} & \tablehead{Final avg. loss $\downarrow$} & \tablehead{Past forgetting $\downarrow$} & \tablehead{Final-task loss $\downarrow$}\\
\midrule
Hard replay & Forward & $\underline{0.719}_{\pm0.192}$ & $\underline{0.075}_{\pm0.101}$ & $1.136_{\pm0.316}$\\
Stored real replay & Forward & $1.090_{\pm0.510}$ & $0.297_{\pm0.315}$ & $1.627_{\pm0.999}$\\
\rowcolor{tableline}
\textbf{Ours} & Forward & $\mathbf{0.527}_{\pm0.132}$ & $\mathbf{0.004}_{\pm0.073}$ & $0.703_{\pm0.268}$\\
\midrule
Hard replay & Reverse & $\underline{0.710}_{\pm0.147}$ & $\underline{0.294}_{\pm0.113}$ & $0.747_{\pm0.236}$\\
Stored real replay & Reverse & $0.913_{\pm0.411}$ & $0.312_{\pm0.244}$ & $1.180_{\pm0.410}$\\

\rowcolor{tableline}
\textbf{Ours} & Reverse & $\mathbf{0.438}_{\pm0.093}$ & $\mathbf{0.116}_{\pm0.271}$ & $0.317_{\pm0.226}$\\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/cagd_per_task.tex <==
\begin{table}[h]
\centering
\caption{Four-task learned-time $\rightarrow$ final held-out loss, averaged
over seeds.  Parentheses give forgetting; columns follow encounter order.}
\label{tab:cagd-per-task}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrrrr}
\toprule
\tablehead{Order} & \tablehead{Method} & \tablehead{Task 1} & \tablehead{Task 2} & \tablehead{Task 3} & \tablehead{Task 4}\\
\midrule
Forward & Sequential & $0.71\!\to\!5.71\ (+5.00)$ & $0.46\!\to\!1.49\ (+1.03)$ & $2.32\!\to\!4.07\ (+1.74)$ & $0.44\!\to\!0.44$\\
\rowcolor{tableline}
\cellcolor{white}
Forward & \CAGD & $\mathbf{0.71\!\to\!1.52\ (+0.81)}$ & $\mathbf{0.36\!\to\!0.58\ (+0.22)}$ & $\mathbf{1.05\!\to\!2.04\ (+0.99)}$ & $\mathbf{0.32\!\to\!0.32}$\\
Reverse & Sequential & $0.35\!\to\!2.12\ (+1.77)$ & $0.64\!\to\!4.31\ (+3.67)$ & $0.53\!\to\!1.09\ (+0.56)$ & $1.16\!\to\!1.16$\\
\rowcolor{tableline}
\cellcolor{white}
Reverse & \CAGD & $\mathbf{0.35\!\to\!0.41\ (+0.06)}$ & $\mathbf{0.55\!\to\!1.75\ (+1.20)}$ & $\mathbf{0.41\!\to\!0.67\ (+0.26)}$ & $\mathbf{0.74\!\to\!0.74}$\\
\bottomrule
\end{tabular}}
\end{table}


==> inputs/tables/cagd_qualitative_additional.tex <==
\begin{table}[H]
\centering
\caption{GSM8K outputs after the \emph{GSM8K $\rightarrow$ summarization $\rightarrow$
creative-writing} stream.  To expose the mixed aggregate result rather than
select only gains, rows are the lowest test indices in three strata among
questions answered correctly when learned: both methods correct,
Sequential-only correct, and \CAGD{}-only correct.  The left column
instantiates the input and target templates; the original rationale is elided
for space. Model: SMDM-219M}
\label{tab:smdm-gsm8k-examples}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}p{0.22\textwidth}p{0.36\textwidth}p{0.36\textwidth}@{}}
\toprule
\tablehead{Input and target} & \tablehead{Sequential final output} & \tablehead{\CAGD{} final output}\\
\midrule
\texttt{Question:} A water tank is filled with 120 liters of water. Celine used 90 liters of
water from the tank to water her small garden. She was then able to collect
rainwater that is twice as much as what was left. How many liters of water are
in the tank now?\par
\texttt{Answer:}\par\smallskip
\textbf{Target template}\par
\texttt{<original rationale>}\par
\texttt{\#\#\#\# 90}
& \emph{Parsed: 90 (correct).} The tank is full of water. The water is very
hot, and she used 90 liters of water. The water is not very hot, and she is
not able to soak the water. Her rainwater is twice as full, and she is now
able to\ldots
& \emph{Parsed: 90 (correct).} The water tank is filled with 120 liters of
water. The water is 90 liters of water. The water is 90 liters of water. The
water is 90 liters of water. The water is 90 liters of water. The water is 90
liters of water.\\
\addlinespace
\texttt{Question:} Lindsay is doing the laundry, and thinks she has missed some socks. There are
50 socks that need washing. If she washes 10 pairs of socks and 15 loose
socks, how many socks has Lindsay missed?\par
\texttt{Answer:}\par\smallskip
\textbf{Target template}\par
\texttt{<original rationale>}\par
\texttt{\#\#\#\# 15}
& \emph{Parsed: 15 (correct).} Lindsay has missed 50 socks. Lindsay washed 10
pairs of socks and 15 loose socks. Lindsay washed 10 pairs of socks and 15
loose socks. Lindsay has missed Lindsay's sock, which is also full of loose
socks. Lindsay has missed Lindsay's sock, which is also\ldots
& \underline{\emph{Parsed: 10 (incorrect).}} Lindsay washes 10 pairs of socks and 15
loose socks. So she washes 10 pairs of socks and 15 loose socks. So she
washes 10 pairs of socks and 15 loose socks. So she washes 10 pairs of socks
and 15 loose socks. So she\ldots\\
\addlinespace
\texttt{Question:} Jared is trying to increase his typing speed. He starts with 47 words per
minute (WPM). After some lessons the next time he tests his typing speed it
has increased to 52 WPM. If he continues to increase his typing speed once
more by 5 words, what will be the average of the three measurements?\par
\texttt{Answer:}\par\smallskip
\textbf{Target template}\par
\texttt{<original rationale>}\par
\texttt{\#\#\#\# 52}
& \emph{Parsed: none (incorrect).} Jared is trying to increase his typing
speed. The first way is to increase his typing speed. The second way is to
increase his typing speed. The third way is to increase his typing speed. The
fourth way is to increase his typing speed. The\ldots
& \textbf{\emph{Parsed: 52 (correct).}} First he will increase his typing speed by 47
words per minute. Then he will increase his typing speed by 52 words per
minute. Then he will increase his typing speed by 52 words per minute.
Finally he will increase his typing speed by 52\ldots\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{Final held-out \emph{summarization} outputs
after the \emph{closed QA $\rightarrow$ summarization $\rightarrow$
creative-writing} stream. The three IDs were fixed from their inputs before
generation. Full prompts, references, and unedited outputs are retained in
the qualitative artifacts.  The left column shows the exact input template
and dataset target. Model: Qwen3-0.6B}
\label{tab:qwen-summarization-examples}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}p{0.28\textwidth}p{0.33\textwidth}p{0.33\textwidth}@{}}
\toprule
\tablehead{Input and target} & \tablehead{Sequential final output} & \tablehead{\CAGD{} final output}\\
\midrule
\texttt{Instruction:} What is dhollywood?\par
\texttt{Context:} Gujarati cinema, also known
as Dhollywood, is the Gujarati language film industry. It is one of the major
regional and vernacular film industries of the cinema of India, having
produced more than one thousand films since its inception.\par
\texttt{Response:}\par\smallskip
\textbf{Target}\par
Dhollywood is a nickname for movies made by Gujarati cinema in India.
& Dhollywood is a fictional story. Dhollywood is a fictional story.
Dhollywood is a fictional story. Dhollywood is a fictional story. Dhollywood
is a fictional story. Dhollywood is a fictional story. Dhollywood is a
fictional story. Dhollywood is a fictional story.
& \textbf{Dhollywood is a nickname for Gujarati cinema.}\\
\addlinespace
\texttt{Instruction:} Please give me the list of airports that are owned by
Australia Pacific Airports Corporation.\par
\texttt{Context:} Australia Pacific Airports
Corporation Limited (APAC) is an unlisted company and owner of two Australian
airports: Melbourne Airport and Launceston Airport. Each airport is operated
by an airport lessee company, in which APAC has a controlling interest:
Australia Pacific Airports (Melbourne) Pty Ltd and Australia Pacific Airports
(Launceston) Pty Ltd respectively.\par
\texttt{Response:}\par\smallskip
\textbf{Target}\par
Australia Pacific Airports
Corporation Limited owns two airports in Australia called Launceston Airport
and Melbourne Airport.
& The purpose of this query is to find out the airports that are owned by the
corporation. The cities of interest are: 38 and 39.
& \textbf{The company has a controlling interest in: 1. Melbourne Airport and 2.
Launceston Airport.}\\
\addlinespace
\texttt{Instruction:} How many people attended the Summer Breeze Open Air?\par
\texttt{Context:} Summer Breeze Open Air is an annual German heavy metal music
festival. It was first held in 1997. The festival had been held in
Abtsgm\"und until 2006 when it was moved to its new location of
Dinkelsb\"uhl, Bavaria. The festival draws around 40,000 attendees annually.
\par\texttt{Response:}\par\smallskip
\textbf{Target}\par
The German heavy metal music festival Summer Breeze Open Air drew 40,000
attendees annually.
& Summer Breeze has an effect on the number of people who attended the
festival. While effect is attribute of effect, effect is attribute of effect.
& Summer Breeze was held in Dinkelsb\"uhl, Bavaria.\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{Final held-out \emph{creative-writing} outputs
from the same model pair and natural-task stream as
\cref{tab:qwen-summarization-examples}.  The task is open-ended, so the table
shows instruction following rather than treating the dataset response as a
unique correct target.  The left column shows the exact input template and
dataset target. Model: Qwen3-0.6B.}
\label{tab:qwen-writing-examples}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}p{0.30\textwidth}p{0.32\textwidth}p{0.32\textwidth}@{}}
\toprule
\tablehead{Input and target} & \tablehead{Sequential final output} & \tablehead{\CAGD{} final output}\\
\midrule
\texttt{Instruction:} Write a dialogue between two hikers, John and Jane, who are lost in the woods
and can't decide what to do. End the argument with Jane winning and them
deciding to turn around and retrace their steps.\par
\texttt{Response:}\par\smallskip
\textbf{Target}\par
John: I think we're lost, this trail doesn't look familiar\newline
Jane: I think you're right. We must have taken a wrong turn at the fork a mile
back. Let's turn around and trace our steps back\newline
John: No, I think we should just keep going forward. We are still on a path,
so we should just go and see if we can find our way back to a path we
know\newline
Jane: I'm worried its going to get dark, and we'll just be going further into
the woods. We should turn around and repeat our steps\newline
John: Okay, you're right. Let's go back to where we first got lost and take the
other side of the fork.
& Before I lost track of time and energy, John and Jane explained their
reasons for being lost and the conversation went through. They agreed upon a
way to proceed and Jane suggested a way to find the way home.
& The last exchange is a conditional. The conditional is conditional on
Jane's last word.\\
\addlinespace
\texttt{Instruction:} Write a poem about George Washington.\par
\texttt{Response:}\par\smallskip
\textbf{Target}\par
George Washington was a British man\newline
The British had laws he couldn't understand\newline
Washington and his friends put together a plan\newline
That the people would resist and America could stand
& The last man on earth, he still stands, he still sees what we do in here,
he still sees what I've done in here, I'll keep on going, I'll keep on going,
I'll keep on going, I'll keep on going, I'll keep on going, I'll\ldots
& The last man on earth, he was the father of our nation, the origin of our
government, the inspiration of our nation. I am amazed by the greatness of
our nation. I hope to visit the country one day and witness the greatness of
our\ldots\\
\addlinespace
\texttt{Instruction:} Write me a thank you note for my high-school teacher\par
\texttt{Response:}\par\smallskip
\textbf{Target}\par
Thank you for being a supportive teacher and encouraging me to keep learning.
I will always remember your encouragement as I move forward in my studies.
& Hi, I hope you have been in good health! I'm so excited to inform you that
I'm almost finished my first year in my major field of interest. I'm so
excited to inform you that I'm almost finished my first year in my major
field\ldots
& The teacher's name, Nick, is a huge part of this note. He's a huge part of
all of us, from when we were kids to today, he's been a huge part in our
education and in our growth. I hope to continue to be in\ldots\\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/fresh_main.tex <==
\begin{table}[t]
\centering
\caption{Continual-learning endpoints (mean $\pm$ SEM over three paired seeds). Past-task forgetting excludes the final task.}
\label{tab:fresh-main}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
\toprule
Order & Method & Final avg. loss $\downarrow$ & Past forgetting $\downarrow$ & Final-task loss $\downarrow$\\
\midrule
Forward & Sequential & $2.445_{\pm 0.524}$ & $+2.678_{\pm 0.783}$ & $0.985_{\pm 0.105}$ \\
Forward & GD & $0.527_{\pm 0.132}$ & $+0.004_{\pm 0.073}$ & $0.703_{\pm 0.268}$ \\
Forward & Rank-1 + GD & $0.590_{\pm 0.252}$ & $+0.006_{\pm 0.117}$ & $0.885_{\pm 0.570}$ \\
Forward & Diagonal + GD & $0.854_{\pm 0.287}$ & $+0.049_{\pm 0.101}$ & $1.602_{\pm 0.664}$ \\
Reverse & Sequential & $2.920_{\pm 0.220}$ & $+3.413_{\pm 0.302}$ & $1.025_{\pm 0.445}$ \\
Reverse & GD & $0.438_{\pm 0.093}$ & $+0.116_{\pm 0.271}$ & $0.317_{\pm 0.226}$ \\
Reverse & Rank-1 + GD & $0.371_{\pm 0.055}$ & $+0.073_{\pm 0.179}$ & $0.206_{\pm 0.090}$ \\
Reverse & Diagonal + GD & $0.553_{\pm 0.141}$ & $+0.242_{\pm 0.262}$ & $0.401_{\pm 0.294}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/fresh_mechanism.tex <==
\begin{table}[t]
\centering
\caption{Final-stage optimization diagnostics. Current, GD, and EWC are weighted per-step objective components; clip is the fraction of steps whose pre-clip gradient norm exceeded 1.}
\label{tab:fresh-mechanism}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrr}
\toprule
Order & Method & Current & GD & EWC & Clip fraction\\
\midrule
Forward & Sequential & $0.025_{\pm 0.002}$ & $0.000_{\pm 0.000}$ & $0$ & $0.068_{\pm 0.009}$ \\
Forward & GD & $0.021_{\pm 0.002}$ & $0.067_{\pm 0.003}$ & $0$ & $0.936_{\pm 0.008}$ \\
Forward & Rank-1 + GD & $0.023_{\pm 0.001}$ & $0.050_{\pm 0.001}$ & $4.55_{\pm 2.89}\!\times\!10^{-2}$ & $0.980_{\pm 0.018}$ \\
Forward & Diagonal + GD & $0.023_{\pm 0.002}$ & $0.067_{\pm 0.004}$ & $8.49_{\pm 3.74}\!\times\!10^{-7}$ & $0.929_{\pm 0.004}$ \\
Reverse & Sequential & $0.026_{\pm 0.002}$ & $0.000_{\pm 0.000}$ & $0$ & $0.111_{\pm 0.004}$ \\
Reverse & GD & $0.013_{\pm 0.001}$ & $0.064_{\pm 0.003}$ & $0$ & $0.930_{\pm 0.023}$ \\
Reverse & Rank-1 + GD & $0.015_{\pm 0.002}$ & $0.061_{\pm 0.006}$ & $9.14_{\pm 7.54}\!\times\!10^{-3}$ & $0.966_{\pm 0.024}$ \\
Reverse & Diagonal + GD & $0.013_{\pm 0.001}$ & $0.067_{\pm 0.003}$ & $1.35_{\pm 0.86}\!\times\!10^{-6}$ & $0.946_{\pm 0.018}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/fresh_per_task.tex <==
\begin{table}[t]
\centering
\caption{Per-task learned-time $\to$ final held-out loss (forgetting), averaged over seeds. Columns follow the encountered order.}
\label{tab:fresh-per-task}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{llrrr}
\toprule
Order & Method & Task 1 & Task 2 & Task 3\\
\midrule
Forward & Sequential & $0.61\!\to\!5.14\ (+4.53)$ & $0.38\!\to\!1.21\ (+0.83)$ & $0.99\!\to\!0.99\ (+0.00)$ \\
Forward & GD & $0.61\!\to\!0.50\ (-0.11)$ & $0.26\!\to\!0.38\ (+0.12)$ & $0.70\!\to\!0.70\ (+0.00)$ \\
Forward & Rank-1 + GD & $0.61\!\to\!0.57\ (-0.04)$ & $0.26\!\to\!0.31\ (+0.05)$ & $0.89\!\to\!0.89\ (+0.00)$ \\
Forward & Diagonal + GD & $0.61\!\to\!0.67\ (+0.06)$ & $0.25\!\to\!0.30\ (+0.04)$ & $1.60\!\to\!1.60\ (+0.00)$ \\
Reverse & Sequential & $0.51\!\to\!7.03\ (+6.52)$ & $0.40\!\to\!0.71\ (+0.30)$ & $1.02\!\to\!1.02\ (+0.00)$ \\
Reverse & GD & $0.51\!\to\!0.60\ (+0.10)$ & $0.26\!\to\!0.39\ (+0.14)$ & $0.32\!\to\!0.32\ (+0.00)$ \\
Reverse & Rank-1 + GD & $0.51\!\to\!0.58\ (+0.08)$ & $0.25\!\to\!0.32\ (+0.07)$ & $0.21\!\to\!0.21\ (+0.00)$ \\
Reverse & Diagonal + GD & $0.51\!\to\!0.92\ (+0.41)$ & $0.27\!\to\!0.34\ (+0.07)$ & $0.40\!\to\!0.40\ (+0.00)$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/fresh_secondary.tex <==
\begin{table}[t]
\centering
\caption{Final behavioral endpoints (mean $\pm$ SEM).}
\label{tab:fresh-secondary}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrr}
\toprule
Order & Method & Token acc. $\uparrow$ & Exact match $\uparrow$ & Containment $\uparrow$ & ROUGE-L $\uparrow$\\
\midrule
Forward & Sequential & $0.430_{\pm 0.082}$ & $0.000_{\pm 0.000}$ & $0.361_{\pm 0.020}$ & $0.174_{\pm 0.013}$ \\
Forward & GD & $0.705_{\pm 0.022}$ & $0.000_{\pm 0.000}$ & $0.644_{\pm 0.006}$ & $0.247_{\pm 0.007}$ \\
Forward & Rank-1 + GD & $0.745_{\pm 0.027}$ & $0.000_{\pm 0.000}$ & $0.628_{\pm 0.022}$ & $0.210_{\pm 0.011}$ \\
Forward & Diagonal + GD & $0.699_{\pm 0.025}$ & $0.000_{\pm 0.000}$ & $0.589_{\pm 0.055}$ & $0.222_{\pm 0.043}$ \\
Reverse & Sequential & $0.456_{\pm 0.022}$ & $0.000_{\pm 0.000}$ & $0.350_{\pm 0.010}$ & $0.181_{\pm 0.018}$ \\
Reverse & GD & $0.699_{\pm 0.069}$ & $0.000_{\pm 0.000}$ & $0.600_{\pm 0.067}$ & $0.186_{\pm 0.023}$ \\
Reverse & Rank-1 + GD & $0.717_{\pm 0.054}$ & $0.000_{\pm 0.000}$ & $0.628_{\pm 0.103}$ & $0.183_{\pm 0.034}$ \\
Reverse & Diagonal + GD & $0.664_{\pm 0.054}$ & $0.000_{\pm 0.000}$ & $0.628_{\pm 0.097}$ & $0.182_{\pm 0.041}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/geometry_summary.tex <==
\begin{table}[t]
\centering
\caption{Held-out geometry at maximum calibration size.  $r$ is the
geometric-mean ratio $e_{\mathrm{rank1}}/e_{\mathrm{diag}}$.
Intervals are 95\% Student-$t$ intervals over probe-seed grid means.}
\label{tab:geometry-main}
\small
\setlength{\tabcolsep}{4.2pt}
\begin{tabular}{llrrrr}
\toprule
Model & Mask evaluation & Mean $s$ & 95\% CI & $r$ $\downarrow$ & Cells won\\
\midrule
219M & fixed grid & $0.086$ & $[0.066,0.106]$ & $0.917$ & 6/15\\
1.14B & fixed grid & $-0.212$ & $[-0.494,0.070]$ & $1.237$ & 3/15\\
219M & uniform-$p$ diagnostic & $-0.009$ & $[-0.036,0.019]$ & $1.009$ & 2/3\\
1.14B & uniform-$p$ diagnostic & $-0.104$ & $[-0.269,0.061]$ & $1.110$ & 0/3\\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/qwen_cagd.tex <==
\begin{table}[t]
\centering
\caption{Full-parameter AR adaptation (mean $\pm$ SEM over three paired seeds), with the archived last-block 4B control separated. Parameter scale is not a controlled intervention.}
\label{tab:qwen-cagd}
\scriptsize
\setlength{\tabcolsep}{3.8pt}
\begin{tabular}{llrr}
\toprule
Qwen3 & Method & Final avg. loss $\downarrow$ & Past forgetting $\downarrow$\\
\midrule
0.6B & Sequential & $3.218_{\pm0.206}$ & $0.434_{\pm0.340}$\\
 & \CAGD & $\mathbf{2.316}_{\pm0.190}$ & $\mathbf{-0.624}_{\pm0.078}$\\
1.7B & Sequential & $2.993_{\pm0.131}$ & $-0.073_{\pm0.144}$\\
 & \CAGD & $\mathbf{2.860}_{\pm0.114}$ & $\mathbf{-0.214}_{\pm0.198}$\\
\midrule
\multicolumn{4}{l}{\emph{Archived last-block control (not rerun)}}\\
4B   & Sequential & $3.996_{\pm0.147}$ & $2.009_{\pm0.159}$\\
     & \CAGD      & $2.797_{\pm0.029}$ & $0.373_{\pm0.058}$\\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r16_main.tex <==
\begin{table}[t]
\centering
\caption{Continual-learning endpoints (mean $\pm$ SEM over three paired seeds). Past-task forgetting excludes the final task.}
\label{tab:r16-main}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
\toprule
Order & Method & Final avg. loss $\downarrow$ & Past forgetting $\downarrow$ & Final-task loss $\downarrow$\\
\midrule
Forward & Sequential & $2.927_{\pm 0.231}$ & $+2.591_{\pm 0.429}$ & $0.439_{\pm 0.039}$ \\
Forward & GD & $1.114_{\pm 0.374}$ & $+0.674_{\pm 0.387}$ & $0.318_{\pm 0.014}$ \\
Forward & Rank-1 & $2.189_{\pm 0.408}$ & $+1.942_{\pm 0.460}$ & $0.357_{\pm 0.046}$ \\
Forward & Diagonal & $3.131_{\pm 0.282}$ & $+2.793_{\pm 0.356}$ & $0.426_{\pm 0.037}$ \\
Forward & Rank-1 + GD & $0.982_{\pm 0.251}$ & $+0.194_{\pm 0.111}$ & $0.948_{\pm 0.645}$ \\
Forward & Diagonal + GD & $0.837_{\pm 0.137}$ & $+0.441_{\pm 0.206}$ & $0.306_{\pm 0.019}$ \\
Forward & Joint & $0.805_{\pm 0.193}$ & -- & -- \\
Reverse & Sequential & $2.168_{\pm 0.390}$ & $+1.997_{\pm 0.395}$ & $1.163_{\pm 0.380}$ \\
Reverse & GD & $0.891_{\pm 0.215}$ & $+0.505_{\pm 0.106}$ & $0.738_{\pm 0.314}$ \\
Reverse & Rank-1 + GD & $0.606_{\pm 0.133}$ & $+0.289_{\pm 0.078}$ & $0.578_{\pm 0.190}$ \\
Reverse & Diagonal + GD & $0.782_{\pm 0.172}$ & $+0.412_{\pm 0.111}$ & $0.621_{\pm 0.210}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r16_mechanism.tex <==
\begin{table}[t]
\centering
\caption{Final-stage optimization diagnostics. Current, GD, and EWC are weighted per-step objective components; clip is the fraction of steps whose pre-clip gradient norm exceeded 1.}
\label{tab:r16-mechanism}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrr}
\toprule
Order & Method & Current & GD & EWC & Clip fraction\\
\midrule
Forward & Sequential & $0.054_{\pm 0.003}$ & $0.000_{\pm 0.000}$ & $0$ & $0.125_{\pm 0.009}$ \\
Forward & GD & $0.055_{\pm 0.003}$ & $0.046_{\pm 0.003}$ & $0$ & $0.921_{\pm 0.003}$ \\
Forward & Rank-1 + GD & $1.171_{\pm 0.972}$ & $0.017_{\pm 0.010}$ & $1.10_{\pm 1.10}\!\times\!10^{3}$ & $0.978_{\pm 0.022}$ \\
Forward & Diagonal + GD & $0.054_{\pm 0.003}$ & $0.044_{\pm 0.002}$ & $1.66_{\pm 0.84}\!\times\!10^{-3}$ & $0.921_{\pm 0.009}$ \\
Reverse & Sequential & $0.040_{\pm 0.006}$ & $0.000_{\pm 0.000}$ & $0$ & $0.128_{\pm 0.022}$ \\
Reverse & GD & $0.028_{\pm 0.003}$ & $0.030_{\pm 0.002}$ & $0$ & $0.864_{\pm 0.026}$ \\
Reverse & Rank-1 + GD & $0.254_{\pm 0.225}$ & $0.018_{\pm 0.007}$ & $1.11_{\pm 1.11}\!\times\!10^{2}$ & $0.988_{\pm 0.009}$ \\
Reverse & Diagonal + GD & $0.029_{\pm 0.003}$ & $0.032_{\pm 0.001}$ & $5.49_{\pm 4.82}\!\times\!10^{-5}$ & $0.869_{\pm 0.012}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r16_per_task.tex <==
\begin{table}[t]
\centering
\caption{Per-task learned-time $\to$ final held-out loss (forgetting), averaged over seeds. Columns follow the encountered order.}
\label{tab:r16-per-task}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{llrrrr}
\toprule
Order & Method & Task 1 & Task 2 & Task 3 & Task 4\\
\midrule
Forward & Sequential & $0.71\!\to\!5.71\ (+5.00)$ & $0.46\!\to\!1.49\ (+1.03)$ & $2.32\!\to\!4.07\ (+1.74)$ & $0.44\!\to\!0.44\ (+0.00)$ \\
Forward & GD & $0.71\!\to\!1.52\ (+0.81)$ & $0.36\!\to\!0.58\ (+0.22)$ & $1.05\!\to\!2.04\ (+0.99)$ & $0.32\!\to\!0.32\ (+0.00)$ \\
Forward & Rank-1 + GD & $0.71\!\to\!0.90\ (+0.19)$ & $0.36\!\to\!0.46\ (+0.11)$ & $1.33\!\to\!1.61\ (+0.28)$ & $0.95\!\to\!0.95\ (+0.00)$ \\
Forward & Diagonal + GD & $0.71\!\to\!0.99\ (+0.28)$ & $0.36\!\to\!0.60\ (+0.25)$ & $0.65\!\to\!1.44\ (+0.79)$ & $0.31\!\to\!0.31\ (+0.00)$ \\
Reverse & Sequential & $0.35\!\to\!2.12\ (+1.77)$ & $0.64\!\to\!4.31\ (+3.67)$ & $0.53\!\to\!1.09\ (+0.56)$ & $1.16\!\to\!1.16\ (+0.00)$ \\
Reverse & GD & $0.35\!\to\!0.41\ (+0.06)$ & $0.55\!\to\!1.75\ (+1.20)$ & $0.41\!\to\!0.67\ (+0.26)$ & $0.74\!\to\!0.74\ (+0.00)$ \\
Reverse & Rank-1 + GD & $0.35\!\to\!0.35\ (-0.00)$ & $0.25\!\to\!1.05\ (+0.80)$ & $0.38\!\to\!0.45\ (+0.07)$ & $0.58\!\to\!0.58\ (+0.00)$ \\
Reverse & Diagonal + GD & $0.35\!\to\!0.36\ (+0.01)$ & $0.53\!\to\!1.55\ (+1.02)$ & $0.40\!\to\!0.60\ (+0.20)$ & $0.62\!\to\!0.62\ (+0.00)$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r16_secondary.tex <==
\begin{table}[t]
\centering
\caption{Final behavioral endpoints (mean $\pm$ SEM).}
\label{tab:r16-secondary}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrr}
\toprule
Order & Method & Token acc. $\uparrow$ & Exact match $\uparrow$ & Containment $\uparrow$ & ROUGE-L $\uparrow$\\
\midrule
Forward & Sequential & $0.436_{\pm 0.041}$ & $0.000_{\pm 0.000}$ & $0.269_{\pm 0.006}$ & $0.241_{\pm 0.013}$ \\
Forward & GD & $0.650_{\pm 0.023}$ & $0.000_{\pm 0.000}$ & $0.494_{\pm 0.027}$ & $0.241_{\pm 0.029}$ \\
Forward & Rank-1 & $0.507_{\pm 0.059}$ & $0.000_{\pm 0.000}$ & $0.367_{\pm 0.071}$ & $0.306_{\pm 0.016}$ \\
Forward & Diagonal & $0.399_{\pm 0.031}$ & $0.000_{\pm 0.000}$ & $0.258_{\pm 0.009}$ & $0.246_{\pm 0.001}$ \\
Forward & Rank-1 + GD & $0.580_{\pm 0.062}$ & $0.000_{\pm 0.000}$ & $0.469_{\pm 0.033}$ & $0.227_{\pm 0.013}$ \\
Forward & Diagonal + GD & $0.610_{\pm 0.024}$ & $0.000_{\pm 0.000}$ & $0.471_{\pm 0.022}$ & $0.230_{\pm 0.029}$ \\
Forward & Joint & $0.788_{\pm 0.006}$ & $0.000_{\pm 0.000}$ & $0.575_{\pm 0.014}$ & $0.371_{\pm 0.003}$ \\
Reverse & Sequential & $0.332_{\pm 0.035}$ & $0.000_{\pm 0.000}$ & $0.292_{\pm 0.023}$ & $0.202_{\pm 0.041}$ \\
Reverse & GD & $0.577_{\pm 0.045}$ & $0.000_{\pm 0.000}$ & $0.300_{\pm 0.034}$ & $0.216_{\pm 0.010}$ \\
Reverse & Rank-1 + GD & $0.683_{\pm 0.054}$ & $0.000_{\pm 0.000}$ & $0.256_{\pm 0.054}$ & $0.212_{\pm 0.012}$ \\
Reverse & Diagonal + GD & $0.598_{\pm 0.051}$ & $0.000_{\pm 0.000}$ & $0.344_{\pm 0.070}$ & $0.234_{\pm 0.007}$ \\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r18_continual_geometry.tex <==
\begin{table}[h!]
\centering
\caption{Full-parameter Fisher reconstruction on the actual first continual
task.  Calibration and test use 40 disjoint prompts and independent masks.
$E_{\mathrm{R1}}$ and $E_{\mathrm{D}}$ score the stored rank-1 and diagonal
surrogates.  $E_{\mathrm{dir}}^*$ keeps the calibration direction but refits
its scalar on test; $E_{\mathrm{best}}^*$ is the best rank-1 fit to the test
Fisher itself.  All $E$ columns are relative Frobenius errors.}
\label{tab:r18-continual-geometry}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{crrrrrrr}
\toprule
Seed & Cal. loss & Test loss & Test/cal. & $E_{\mathrm{R1}}$ & $E_{\mathrm{D}}$ & $E_{\mathrm{dir}}^*$ & $E_{\mathrm{best}}^*$\\
\midrule
3407 & $1.43\!\times\!10^{-4}$ & 0.422 & 2948.8 & 0.999999999848 & 0.999999999997 & 0.999997178 & 0.523869\\
3408 & $1.61\!\times\!10^{-4}$ & 0.627 & 3898.5 & 0.999999999890 & 0.999999999997 & 0.999999517 & 0.318657\\
3409 & $2.43\!\times\!10^{-4}$ & 0.239 & 980.7  & 0.999999987483 & 0.999999999964 & 0.999988531 & 0.496539\\
\midrule
Mean & $1.83\!\times\!10^{-4}$ & 0.429 & 2609.3 & 0.999999995740 & 0.999999999986 & 0.999995075 & 0.446355\\
\bottomrule
\end{tabular}}
\end{table}


==> inputs/tables/r23_trace_endpoints.tex <==
\begin{table}[h!]
\centering
\caption{Exploratory two-task endpoints and mechanism diagnostics under
matched implemented weighted trace.  Loss, clipping, and gradient columns are
mean $\pm$ SEM over three paired seeds.  Gradient
norm is the maximum pre-clip norm in a run; EWC reports the across-seed means
of each run's weighted per-step mean/maximum.}
\label{tab:r23-trace-endpoints}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{clrrrrrr}
\toprule
Clip & Method & Final avg. $\downarrow$ & Past forgetting $\downarrow$ & Final task $\downarrow$ & Clip fraction & Max grad. & EWC mean/max\\
\midrule
1 & GD & $0.666_{\pm0.153}$ & $+0.260_{\pm0.271}$ & $0.361_{\pm0.048}$ & $0.991_{\pm0.001}$ & $290_{\pm18}$ & --\\
1 & Rank-1 + GD & $0.626_{\pm0.192}$ & $+0.173_{\pm0.323}$ & $0.368_{\pm0.032}$ & $0.992_{\pm0.002}$ & $290_{\pm15}$ & $2.95\!\times\!10^{-5}/5.00\!\times\!10^{-4}$\\
1 & Diagonal + GD & $0.625_{\pm0.243}$ & $+0.183_{\pm0.414}$ & $0.357_{\pm0.032}$ & $0.990_{\pm0.001}$ & $301_{\pm10}$ & $1.25\!\times\!10^{-6}/2.00\!\times\!10^{-6}$\\
\midrule
$10^6$ & GD & $0.642_{\pm0.233}$ & $+0.249_{\pm0.395}$ & $0.325_{\pm0.024}$ & 0 & $412_{\pm49}$ & --\\
$10^6$ & Rank-1 + GD & $0.665_{\pm0.216}$ & $+0.305_{\pm0.372}$ & $0.313_{\pm0.026}$ & 0 & $412_{\pm56}$ & $8.85\!\times\!10^{-6}/4.21\!\times\!10^{-4}$\\
$10^6$ & Diagonal + GD & $0.670_{\pm0.217}$ & $+0.310_{\pm0.399}$ & $0.319_{\pm0.026}$ & 0 & $393_{\pm39}$ & $9.00\!\times\!10^{-7}/1.30\!\times\!10^{-6}$\\
\bottomrule
\end{tabular}}
\end{table}


==> inputs/tables/r23_trace_paired.tex <==
\begin{table}[h!]
\centering
\caption{Paired differences for the implemented weighted-trace controls at
SMDM-219M and SMDM-1.14B (mean $\pm$ SEM).  Clip is the gradient-norm clipping
threshold.  Parentheses count seeds below zero out of three; negative values
favor the method named first.}
\label{tab:r23-trace-paired}
\label{tab:r24-trace-paired}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccc@{}}
\toprule
\tablehead{Model} & \tablehead{Clip} & \tablehead{Contrast} & \tablehead{$\Delta$ final avg. $\downarrow$} & \tablehead{$\Delta$ forgetting $\downarrow$} & \tablehead{$\Delta$ final task $\downarrow$}\\
\midrule
 &  & Rank-1 + \textbf{Ours} $-$ \textbf{Ours} & $+0.091_{\pm0.086}$ (1) & $+0.148_{\pm0.168}$ (1) & $+0.033_{\pm0.008}$ (0)\\
 &  & Diagonal + \textbf{Ours} $-$ \textbf{Ours} & $+0.128_{\pm0.068}$ (0) & $+0.251_{\pm0.154}$ (1) & $+0.005_{\pm0.022}$ (1)\\
\multirow{-3}{*}{SMDM-219M} & \multirow{-3}{*}{1} & Rank-1 + \textbf{Ours} $-$ Diagonal + \textbf{Ours} & $-0.038_{\pm0.154}$ (2) & $-0.103_{\pm0.322}$ (2) & $+0.027_{\pm0.024}$ (1)\\
\midrule
 &  & Rank-1 + \textbf{Ours} $-$ \textbf{Ours} & $+0.017_{\pm0.047}$ (2) & $+0.016_{\pm0.110}$ (2) & $+0.018_{\pm0.017}$ (1)\\
 &  & Diagonal + \textbf{Ours} $-$ \textbf{Ours} & $+0.029_{\pm0.093}$ (2) & $+0.041_{\pm0.168}$ (2) & $+0.016_{\pm0.019}$ (2)\\
\multirow{-3}{*}{SMDM-219M} & \multirow{-3}{*}{$10^6$} & Rank-1 + \textbf{Ours} $-$ Diagonal + \textbf{Ours} & $-0.012_{\pm0.121}$ (1) & $-0.025_{\pm0.238}$ (1) & $+0.002_{\pm0.014}$ (2)\\
\midrule
 &  & Rank-1 + \textbf{Ours} $-$ \textbf{Ours} & $-0.693_{\pm0.204}$ (3) & $-1.223_{\pm0.347}$ (3) & $-0.162_{\pm0.112}$ (2)\\
 &  & Diagonal + \textbf{Ours} $-$ \textbf{Ours} & $-0.169_{\pm0.105}$ (2) & $-0.253_{\pm0.172}$ (2) & $-0.086_{\pm0.041}$ (3)\\
\multirow{-3}{*}{SMDM-1.14B} & \multirow{-3}{*}{1} & Rank-1 + \textbf{Ours} $-$ Diagonal + \textbf{Ours} & $-0.523_{\pm0.298}$ (3) & $-0.971_{\pm0.515}$ (3) & $-0.076_{\pm0.112}$ (2)\\
\bottomrule
\end{tabular*}
\end{table}


==> inputs/tables/r24_trace_paired.tex <==
\begin{table}[h!]
\centering
\caption{Paired 1.14B effects (mean $\pm$ SEM).  Parentheses count seeds below
zero out of three; negative values favor the method named first.}
\label{tab:r24-trace-paired}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccc}
\toprule
\tablehead{Contrast} & \tablehead{$\Delta$ final avg. $\downarrow$} & \tablehead{$\Delta$ forgetting $\downarrow$} & \tablehead{$\Delta$ final task $\downarrow$}\\
\midrule
Rank-1 + \textbf{Ours} $-$ \textbf{Ours} & $+0.052_{\pm0.061}$ (2) & $+0.149_{\pm0.147}$ (1) & $-0.044_{\pm0.026}$ (3)\\
Diagonal + \textbf{Ours} $-$ \textbf{Ours} & $-0.028_{\pm0.008}$ (3) & $-0.068_{\pm0.057}$ (3) & $+0.012_{\pm0.041}$ (2)\\
Rank-1 + \textbf{Ours} $-$ Diagonal + \textbf{Ours} & $+0.080_{\pm0.070}$ (0) & $+0.217_{\pm0.204}$ (0) & $-0.057_{\pm0.066}$ (2)\\
\bottomrule
\end{tabular}
\end{table}


==> inputs/tables/r24_trace_scale.tex <==
\begin{table}[h!]
\centering
\caption{Full-parameter 1.14B implemented weighted-trace extension.  The
target is $\tr(\lambda\widehat F)$ and is identical across methods within a
seed; final average losses report all nine cells.  EWC columns are mean
weighted Task-B components.}
\label{tab:r24-trace-scale}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{crrrrrrr}
\toprule
Seed & Trace target & $\lambda_{\mathrm{R1}}$ & GD loss & Rank-1 + GD & Diagonal + GD & Rank-1 EWC & Diagonal EWC\\
\midrule
3407 & $3.7149\!\times\!10^{4}$ & 743.6  & 0.3869 & 0.5620 & 0.3427 & $1.4165\!\times\!10^{2}$ & $3.2965\!\times\!10^{-3}$\\
3408 & 2.5483 & 871.6  & 0.2631 & 0.2523 & 0.2463 & $4.6731\!\times\!10^{-6}$ & $4.2200\!\times\!10^{-7}$\\
3409 & 0.1446 & 2214.0 & 0.2565 & 0.2490 & 0.2334 & $2.7644\!\times\!10^{-6}$ & $2.5564\!\times\!10^{-8}$\\
\bottomrule
\end{tabular}}
\end{table}


==> inputs/tables/two_task.tex <==
\begin{table}[t]
\centering
\caption{Two-task confirmation on separate facts (mean $\pm$ SEM over three paired seeds). Validation selected Rank-1 $\lambda=10^{5}$ and diagonal $\lambda=10^{3}$.}
\label{tab:two-task}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrr}
\toprule
Method & Final average loss $\downarrow$ & Task-A forgetting $\downarrow$ & Task-B loss $\downarrow$\\
\midrule
Sequential & $1.485_{\pm 0.172}$ & $+2.475_{\pm 0.327}$ & $0.389_{\pm 0.062}$ \\
GD & $0.182_{\pm 0.011}$ & $-0.028_{\pm 0.029}$ & $0.285_{\pm 0.012}$ \\
Rank-1 + GD & $0.196_{\pm 0.023}$ & $-0.003_{\pm 0.079}$ & $0.288_{\pm 0.015}$ \\
Diagonal + GD & $0.174_{\pm 0.004}$ & $-0.044_{\pm 0.036}$ & $0.286_{\pm 0.021}$ \\
\bottomrule
\end{tabular}
\end{table}

